Dilaton cosmology and phenomenology

This paper is dedicated to Gabriele Veneziano on his 65th birthday. Most of the results reported here are known results, due to Gabriele, or obtained in collaboration with him, or inspired by our joint work on string cosmology. A few new results are also presented concerning the duality invariance of a non-local dilaton coupling to the matter sources, and its possible cosmological applications in the context of the dark-energy scenario.

==> svind.ist.tex <==
 delim_0 "\\idxquad "
delim_1 "\\idxquad "
delim_2 "\\idxquad "
delim_n ",\\,"

